ACT: Anti-Crosstalk Learning for Cross-Sectional Stock Ranking via Temporal Disentanglement and Structural Purification

Cross-sectional stock ranking is a fundamental task in quantitative investment, relying on both temporal modeling of individual stocks and the capture of inter-stock dependencies. While existing deep learning models leverage graph-based approaches to enhance ranking accuracy by propagating information over relational graphs, they suffer from a key challenge: crosstalk, namely unintended information interference across predictive factors. We identify two forms of crosstalk: temporal-scale crosstalk, where trends, fluctuations, and shocks are entangled in a shared representation and non-transferable local patterns contaminate cross-stock learning; and structural crosstalk, where heterogeneous relations are indiscriminately fused and relation-specific predictive signals are obscured. To address both issues, we propose the Anti-CrossTalk (ACT) framework for cross-sectional stock ranking via temporal disentanglement and structural purification. Specifically, ACT first decomposes each stock sequence into trend, fluctuation, and shock components, then extracts component-specific information through dedicated branches, which effectively decouples non-transferable local patterns. ACT further introduces a Progressive Structural Purification Encoder to sequentially purify structural crosstalk on the trend component after mitigating temporal-scale crosstalk. An adaptive fusion module finally integrates all branch representations for ranking. Experiments on CSI300 and CSI500 demonstrate that ACT achieves state-of-the-art ranking accuracy and superior portfolio performance, with improvements of up to 74.25% on the CSI300 dataset.

==> ff/ff_regression_tables.tex <==
% Auto-generated Fama-French regression tables
% Requires: booktabs, multirow, graphicx, threeparttable packages

\begin{table}[!t]
\centering
\caption{Fama-French factor regression on CSI300.}
\label{tab:ff_regression_csi300}
\renewcommand{\arraystretch}{1.08}
\setlength{\tabcolsep}{3pt}
\footnotesize
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{11}{l}{\textbf{Panel A: Five-Factor Model}} \\
\midrule
\textbf{Model} & $\hat{\alpha}$ (\%) & $t(\alpha)$ & $\beta_{\text{MktRF}}$ & $\beta_{\text{SMB}}$ & $\beta_{\text{HML}}$ & $\beta_{\text{RMW}}$ & $\beta_{\text{CMA}}$ & $R^2$ & $N$ \\
\midrule
\rowcolor{gray!15} \textbf{ACT} & \textbf{24.06***} & \textbf{6.22} & \textbf{0.016} & \textbf{-0.035} & \textbf{0.018} & \textbf{-0.006} & \textbf{0.073} & \textbf{0.019} & \textbf{625} \\
LSTM & 19.60*** & 6.15 & -0.003 & 0.003 & 0.027 & 0.028 & 0.009 & 0.003 & 664 \\
GRU & 19.17*** & 5.94 & 0.012 & -0.021 & -0.003 & 0.011 & 0.026 & 0.006 & 664 \\
ALSTM & 19.51*** & 6.62 & -0.001 & -0.005 & 0.012 & 0.020 & 0.029 & 0.002 & 664 \\
SFM & 19.58*** & 6.33 & 0.003 & -0.004 & 0.018 & 0.007 & 0.042 & 0.005 & 664 \\
TCN & 20.10*** & 6.33 & 0.012 & -0.015 & -0.010 & -0.005 & -0.002 & 0.005 & 664 \\
Transformer & 22.57*** & 6.49 & 0.008 & -0.002 & 0.021 & 0.009 & 0.024 & 0.004 & 664 \\
TabNet & 17.92*** & 5.59 & 0.006 & -0.005 & -0.016 & -0.022 & 0.016 & 0.003 & 664 \\
Localformer & 22.71*** & 7.01 & 0.001 & -0.001 & -0.010 & -0.005 & 0.017 & 0.002 & 664 \\
XGBoost & 8.05*** & 3.18 & -0.005 & -0.005 & -0.002 & 0.020 & 0.002 & 0.003 & 664 \\
CatBoost & 19.43*** & 5.58 & -0.002 & -0.014 & -0.020 & -0.053 & 0.019 & 0.007 & 664 \\
LightGBM & 17.58*** & 5.17 & -0.001 & -0.016 & 0.010 & -0.015 & 0.047 & 0.007 & 664 \\
DoubleEnsemble & 17.38*** & 4.88 & 0.010 & 0.002 & 0.000 & -0.033 & 0.002 & 0.004 & 664 \\
\midrule
\multicolumn{11}{l}{\textbf{Panel B: Three-Factor Model}} \\
\midrule
\textbf{Model} & $\hat{\alpha}$ (\%) & $t(\alpha)$ & $\beta_{\text{MktRF}}$ & $\beta_{\text{SMB}}$ & $\beta_{\text{HML}}$ & \multicolumn{2}{c}{---} & $R^2$ & $N$ \\
\midrule
\rowcolor{gray!15} \textbf{ACT} & \textbf{23.59***} & \textbf{6.00} & \textbf{0.017} & \textbf{-0.014} & \textbf{0.033} & & & \textbf{0.012} & \textbf{625} \\
LSTM & 19.55*** & 6.16 & 0.000 & 0.000 & 0.017 & & & 0.002 & 664 \\
GRU & 19.01*** & 5.94 & 0.014 & -0.015 & -0.003 & & & 0.005 & 664 \\
ALSTM & 19.33*** & 6.67 & 0.002 & -0.001 & 0.008 & & & 0.000 & 664 \\
SFM & 19.31*** & 6.21 & 0.004 & 0.006 & 0.023 & & & 0.002 & 664 \\
TCN & 20.12*** & 6.39 & 0.011 & -0.015 & -0.009 & & & 0.005 & 664 \\
Transformer & 22.42*** & 6.48 & 0.009 & 0.003 & 0.022 & & & 0.003 & 664 \\
TabNet & 17.80*** & 5.53 & 0.004 & 0.004 & -0.003 & & & 0.001 & 664 \\
Localformer & 22.59*** & 6.97 & 0.001 & 0.005 & -0.005 & & & 0.001 & 664 \\
XGBoost & 8.05*** & 3.17 & -0.003 & -0.008 & -0.010 & & & 0.002 & 664 \\
CatBoost & 19.27*** & 5.49 & -0.006 & 0.001 & 0.006 & & & 0.001 & 664 \\
LightGBM & 17.26*** & 5.11 & -0.002 & 0.000 & 0.025 & & & 0.004 & 664 \\
DoubleEnsemble & 17.35*** & 4.83 & 0.007 & 0.009 & 0.015 & & & 0.002 & 664 \\
\bottomrule
\end{tabular}}
\begin{tablenotes}
\footnotesize
\item[] $\hat{\alpha}$ is the annualized alpha (\%). $t$-statistics use Newey-West HAC standard errors (5 lags). ***, **, * denote significance at 1\%, 5\%, 10\% levels.
\end{tablenotes}
\end{table}

\begin{table}[!t]
\centering
\caption{Fama-French factor regression on CSI500.}
\label{tab:ff_regression_csi500}
\renewcommand{\arraystretch}{1.08}
\setlength{\tabcolsep}{3pt}
\footnotesize
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{11}{l}{\textbf{Panel A: Five-Factor Model}} \\
\midrule
\textbf{Model} & $\hat{\alpha}$ (\%) & $t(\alpha)$ & $\beta_{\text{MktRF}}$ & $\beta_{\text{SMB}}$ & $\beta_{\text{HML}}$ & $\beta_{\text{RMW}}$ & $\beta_{\text{CMA}}$ & $R^2$ & $N$ \\
\midrule
\rowcolor{gray!15} \textbf{ACT} & \textbf{59.09***} & \textbf{13.34} & \textbf{-0.001} & \textbf{-0.013} & \textbf{-0.008} & \textbf{-0.019} & \textbf{0.008} & \textbf{0.002} & \textbf{625} \\
LSTM & 23.37*** & 6.67 & -0.009 & 0.015 & -0.012 & -0.016 & -0.006 & 0.005 & 664 \\
GRU & 33.16*** & 8.78 & -0.006 & 0.015 & 0.023 & 0.001 & -0.029 & 0.003 & 664 \\
ALSTM & 37.40*** & 9.31 & -0.003 & 0.007 & 0.034 & 0.024 & 0.006 & 0.003 & 664 \\
SFM & 28.97*** & 8.14 & -0.019 & 0.006 & 0.022 & -0.006 & -0.024 & 0.007 & 664 \\
TCN & 29.60*** & 7.87 & -0.000 & 0.001 & 0.019 & 0.016 & 0.051 & 0.005 & 664 \\
Transformer & 38.04*** & 9.24 & -0.015 & 0.000 & 0.043 & 0.019 & 0.031 & 0.011 & 664 \\
TabNet & 31.13*** & 8.52 & -0.004 & -0.007 & 0.012 & -0.030 & 0.014 & 0.006 & 664 \\
Localformer & 36.86*** & 9.20 & -0.011 & 0.015 & 0.077 & 0.076 & 0.005 & 0.013 & 664 \\
XGBoost & 35.73*** & 8.68 & -0.021 & 0.013 & 0.047 & 0.049 & 0.015 & 0.008 & 664 \\
CatBoost & 29.86*** & 7.08 & -0.022 & -0.008 & -0.005 & 0.046 & 0.027 & 0.005 & 664 \\
LightGBM & 29.57*** & 6.67 & -0.008 & 0.009 & 0.013 & -0.013 & 0.011 & 0.002 & 664 \\
DoubleEnsemble & 32.36*** & 7.21 & 0.000 & -0.012 & 0.046 & 0.040 & 0.083 & 0.011 & 664 \\
\midrule
\multicolumn{11}{l}{\textbf{Panel B: Three-Factor Model}} \\
\midrule
\textbf{Model} & $\hat{\alpha}$ (\%) & $t(\alpha)$ & $\beta_{\text{MktRF}}$ & $\beta_{\text{SMB}}$ & $\beta_{\text{HML}}$ & \multicolumn{2}{c}{---} & $R^2$ & $N$ \\
\midrule
\rowcolor{gray!15} \textbf{ACT} & \textbf{59.05***} & \textbf{13.29} & \textbf{-0.003} & \textbf{-0.008} & \textbf{0.002} & & & \textbf{0.001} & \textbf{625} \\
LSTM & 23.40*** & 6.68 & -0.011 & 0.016 & -0.007 & & & 0.005 & 664 \\
GRU & 33.35*** & 8.88 & -0.007 & 0.006 & 0.017 & & & 0.002 & 664 \\
ALSTM & 37.37*** & 9.26 & -0.001 & 0.004 & 0.025 & & & 0.002 & 664 \\
SFM & 29.12*** & 8.17 & -0.020 & 0.001 & 0.021 & & & 0.007 & 664 \\
TCN & 29.28*** & 7.79 & 0.003 & 0.012 & 0.021 & & & 0.002 & 664 \\
Transformer & 37.84*** & 9.24 & -0.012 & 0.006 & 0.041 & & & 0.009 & 664 \\
TabNet & 31.02*** & 8.54 & -0.006 & 0.003 & 0.028 & & & 0.004 & 664 \\
Localformer & 36.86*** & 9.10 & -0.003 & 0.002 & 0.046 & & & 0.008 & 664 \\
XGBoost & 35.65*** & 8.78 & -0.015 & 0.008 & 0.029 & & & 0.005 & 664 \\
CatBoost & 29.71*** & 7.00 & -0.017 & -0.009 & -0.020 & & & 0.003 & 664 \\
LightGBM & 29.49*** & 6.65 & -0.009 & 0.014 & 0.020 & & & 0.002 & 664 \\
DoubleEnsemble & 31.84*** & 7.03 & 0.006 & 0.004 & 0.044 & & & 0.005 & 664 \\
\bottomrule
\end{tabular}}
\begin{tablenotes}
\footnotesize
\item[] $\hat{\alpha}$ is the annualized alpha (\%). $t$-statistics use Newey-West HAC standard errors (5 lags). ***, **, * denote significance at 1\%, 5\%, 10\% levels.
\end{tablenotes}
\end{table}

\begin{table}[!t]
\centering
\caption{Alpha comparison across models and factor models.}
\label{tab:alpha_summary}
\renewcommand{\arraystretch}{1.08}
\setlength{\tabcolsep}{4pt}
\footnotesize
\begin{tabular}{lcccccccc}
\toprule
 & \multicolumn{4}{c}{\textbf{CSI300}} & \multicolumn{4}{c}{\textbf{CSI500}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
 & \multicolumn{2}{c}{FF3} & \multicolumn{2}{c}{FF5} & \multicolumn{2}{c}{FF3} & \multicolumn{2}{c}{FF5} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
\textbf{Model} & $\hat{\alpha}$(\%) & $t$ & $\hat{\alpha}$(\%) & $t$ & $\hat{\alpha}$(\%) & $t$ & $\hat{\alpha}$(\%) & $t$ \\
\midrule
\textbf{ACT} & \textbf{23.59***} & \textbf{6.00} & \textbf{24.06***} & \textbf{6.22} & \textbf{59.05***} & \textbf{13.29} & \textbf{59.09***} & \textbf{13.34} \\
LSTM & 19.55*** & 6.16 & 19.60*** & 6.15 & 23.40*** & 6.68 & 23.37*** & 6.67 \\
GRU & 19.01*** & 5.94 & 19.17*** & 5.94 & 33.35*** & 8.88 & 33.16*** & 8.78 \\
ALSTM & 19.33*** & 6.67 & 19.51*** & 6.62 & 37.37*** & 9.26 & 37.40*** & 9.31 \\
SFM & 19.31*** & 6.21 & 19.58*** & 6.33 & 29.12*** & 8.17 & 28.97*** & 8.14 \\
TCN & 20.12*** & 6.39 & 20.10*** & 6.33 & 29.28*** & 7.79 & 29.60*** & 7.87 \\
Transformer & 22.42*** & 6.48 & 22.57*** & 6.49 & 37.84*** & 9.24 & 38.04*** & 9.24 \\
TabNet & 17.80*** & 5.53 & 17.92*** & 5.59 & 31.02*** & 8.54 & 31.13*** & 8.52 \\
Localformer & 22.59*** & 6.97 & 22.71*** & 7.01 & 36.86*** & 9.10 & 36.86*** & 9.20 \\
XGBoost & 8.05*** & 3.17 & 8.05*** & 3.18 & 35.65*** & 8.78 & 35.73*** & 8.68 \\
CatBoost & 19.27*** & 5.49 & 19.43*** & 5.58 & 29.71*** & 7.00 & 29.86*** & 7.08 \\
LightGBM & 17.26*** & 5.11 & 17.58*** & 5.17 & 29.49*** & 6.65 & 29.57*** & 6.67 \\
DoubleEnsemble & 17.35*** & 4.83 & 17.38*** & 4.88 & 31.84*** & 7.03 & 32.36*** & 7.21 \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\footnotesize
\item[] $\hat{\alpha}$: annualized alpha (\%). HAC $t$-statistics (Newey-West, 5 lags). ***, **, * denote 1\%, 5\%, 10\% significance.
\end{tablenotes}
\end{table}
